Constructing strongly equivalent nonisomorphic models for unsuperstable theories. Part B

We study how equivalent nonisomorphic models of unsuperstable theories can be. We measure the equivalence by Ehrenfeucht-Fraisse games. This paper continues [HySh:474].

==> mssymb.tex <==

\message{Not using the real mssymb file}
\message{Inputting amssym.def and amssym.tex instead}
 {\catcode`\@11 \global\def\setboxz@h{\setbox0\hbox}
	\global\def\wdz@{\wd0 }
 }

\input amssym.def
\input amssym.tex
\def\napprox{\not\approx}

